Precise Legal Sentence Boundary Detection for Retrieval at Scale: NUPunkt and CharBoundary

We present NUPunkt and CharBoundary, two sentence boundary detection libraries optimized for high-precision, high-throughput processing of legal text in large-scale applications such as due diligence, e-discovery, and legal research. These libraries address the critical challenges posed by legal documents containing specialized citations, abbreviations, and complex sentence structures that confound general-purpose sentence boundary detectors. Our experimental evaluation on five diverse legal datasets comprising over 25,000 documents and 197,000 annotated sentence boundaries demonstrates that NUPunkt achieves 91.1% precision while processing 10 million characters per second with modest memory requirements (432 MB). CharBoundary models offer balanced and adjustable precision-recall tradeoffs, with the large model achieving the highest F1 score (0.782) among all tested methods. Notably, NUPunkt provides a 29-32% precision improvement over general-purpose tools while maintaining exceptional throughput, processing multi-million document collections in minutes rather than hours. Both libraries run efficiently on standard CPU hardware without requiring specialized accelerators. NUPunkt is implemented in pure Python with zero external dependencies, while CharBoundary relies only on scikit-learn and optional ONNX runtime integration for optimized performance. Both libraries are available under the MIT license, can be installed via PyPI, and can be interactively tested at https://sentences.aleainstitute.ai/. These libraries address critical precision issues in retrieval-augmented generation systems by preserving coherent legal concepts across sentences, where each percentage improvement in precision yields exponentially greater reductions in context fragmentation, creating cascading benefits throughout retrieval pipelines and significantly enhancing downstream reasoning quality.

==> Makefile <==
# Configuration
MAIN_TEX := main.tex
OUTPUT_PDF := $(MAIN_TEX:.tex=.pdf)
BIB_FILE := main.bib
LATEX_ENGINE := pdflatex
BIBTEX_ENGINE := bibtex
LATEXMK := latexmk
PYTHON := python

# Directories
FIGURES_DIR := figures
SECTIONS_DIR := sections
TABLES_DIR := tables
RESULTS_DIR := ../results/paper_results_20250402_203406

# Figure generation script (optional)
FIGURE_SCRIPT := ../src/lsp/visualization.py

# Command line options
LATEX_OPTS := -interaction=nonstopmode -halt-on-error
LATEXMK_OPTS := -pdf -bibtex

# Check if we're in verbose mode
ifdef VERBOSE
	QUIET :=
	REDIRECT :=
else
	QUIET := -quiet
	REDIRECT := > /dev/null 2>&1
endif

# Default target - use manual sequence instead of latexmk due to reliability
all: $(OUTPUT_PDF)

# Build using manual sequence which is more reliable
$(OUTPUT_PDF): $(MAIN_TEX) $(wildcard $(SECTIONS_DIR)/*.tex) $(wildcard $(TABLES_DIR)/*.tex) $(wildcard $(FIGURES_DIR)/*.pdf) $(BIB_FILE)
	@echo "Building $(OUTPUT_PDF)..."
	$(LATEX_ENGINE) $(LATEX_OPTS) $(MAIN_TEX)
	$(BIBTEX_ENGINE) $(basename $(MAIN_TEX))
	$(LATEX_ENGINE) $(LATEX_OPTS) $(MAIN_TEX)
	$(LATEX_ENGINE) $(LATEX_OPTS) $(MAIN_TEX)
	@echo "Build complete."

# Alternative build using latexmk (may fail more often)
latexmk:
	@echo "Building with latexmk..."
	$(LATEXMK) $(LATEXMK_OPTS) $(MAIN_TEX)
	@echo "Build complete."

# Copy publication figures from results
figures:
	@echo "Copying publication figures..."
	mkdir -p $(FIGURES_DIR)
	cp $(RESULTS_DIR)/publication_charts/*.pdf $(FIGURES_DIR)/
	@echo "Figures copied."

# Copy LaTeX tables from results directory
tables:
	@echo "Copying LaTeX tables..."
	mkdir -p $(TABLES_DIR)
	cp $(RESULTS_DIR)/latex/*.tex $(TABLES_DIR)/
	# Fix underscores in table files
	# sed -i 's/alea_train/ALEA Train/g; s/multilegal_scotus/SCOTUS/g; s/multilegal_cyber_crime/Cyber Crime/g; s/multilegal_bva/BVA/g; s/multilegal_intellectual_property/Intellectual Property/g' $(TABLES_DIR)/dataset_stats_table.tex
	# sed -i 's/alea_train/ALEA Train/g; s/multilegal_scotus/SCOTUS/g; s/multilegal_cyber_crime/Cyber Crime/g; s/multilegal_bva/BVA/g; s/multilegal_intellectual_property/Intellectual Property/g; s/charboundary_/charboundary-/g; s/nltk_punkt/nltk punkt/g; s/spacy_sm/spaCy (sm)/g; s/spacy_lg/spaCy (lg)/g; s/pysbd/pySBD/g' $(TABLES_DIR)/performance_table.tex
	@echo "Tables copied and fixed."

# View the compiled PDF
view: $(OUTPUT_PDF)
	@echo "Opening $(OUTPUT_PDF)..."
	@if command -v xdg-open > /dev/null; then \
		xdg-open $(OUTPUT_PDF); \
	elif command -v open > /dev/null; then \
		open $(OUTPUT_PDF); \
	else \
		echo "Could not find a program to open $(OUTPUT_PDF)"; \
	fi

# Clean temporary files
clean:
	@echo "Cleaning temporary files..."
	rm -f *.aux *.bbl *.blg *.log *.out *.toc *.lof *.lot *.fls *.fdb_latexmk *.synctex.gz
	@echo "Clean complete."

# Full rebuild
rebuild: clean all

# Prepare assets (figures and tables)
prepare: figures tables

# Complete build process including assets
full: clean prepare 
	@echo "Running full build with complete sequence..."
	$(LATEX_ENGINE) $(LATEX_OPTS) $(MAIN_TEX)
	$(BIBTEX_ENGINE) $(basename $(MAIN_TEX))
	$(LATEX_ENGINE) $(LATEX_OPTS) $(MAIN_TEX)
	$(LATEX_ENGINE) $(LATEX_OPTS) $(MAIN_TEX)
	@echo "Full build complete."

# Check status of required directories and files
check:
	@echo "Checking paper structure..."
	@mkdir -p $(FIGURES_DIR) $(TABLES_DIR)
	@echo "Main tex file: $(shell [ -f $(MAIN_TEX) ] && echo 'Found' || echo 'Missing')"
	@echo "Bibliography file: $(shell [ -f $(BIB_FILE) ] && echo 'Found' || echo 'Missing')"
	@echo "Sections directory: $(shell [ -d $(SECTIONS_DIR) ] && echo 'Found' || echo 'Missing')"
	@echo "Tables directory: $(shell [ -d $(TABLES_DIR) ] && echo 'Found' || echo 'Missing')"
	@echo "Figures directory: $(shell [ -d $(FIGURES_DIR) ] && echo 'Found' || echo 'Missing')"
	@echo "Section files found: $(shell ls -1 $(SECTIONS_DIR)/*.tex 2>/dev/null | wc -l)"
	@echo "Table files found: $(shell ls -1 $(TABLES_DIR)/*.tex 2>/dev/null | wc -l)"
	@echo "Figure files found: $(shell ls -1 $(FIGURES_DIR)/*.pdf 2>/dev/null | wc -l)"

# Help target
help:
	@echo "Legal Sentence Boundary Detection Paper Makefile"
	@echo ""
	@echo "Available targets:"
	@echo "  all       - Build the PDF using manual sequence (default target)"
	@echo "  latexmk   - Build using latexmk (alternative)"
	@echo "  clean     - Remove temporary files"
	@echo "  rebuild   - Clean and rebuild"
	@echo "  view      - Open the PDF with default viewer"
	@echo "  figures   - Copy publication figures from results"
	@echo "  tables    - Copy LaTeX tables from results"
	@echo "  prepare   - Copy all assets (figures and tables)"
	@echo "  full      - Complete build including asset copying"
	@echo "  check     - Check paper structure and required files"
	@echo ""
	@echo "Options:"
	@echo "  VERBOSE=1 - Show detailed build output"

# Phony targets
.PHONY: all latexmk clean rebuild view figures tables prepare full check help


==> tables/main_results_table.tex <==
\begin{table}[htbp]
\centering
\caption{Performance and Resource Efficiency of Sentence Boundary Detection Methods}
\label{tab:main-results}
\begin{tabular}{lrrrr}
\toprule
\textbf{Model} & \textbf{Precision} & \textbf{F1} & \textbf{Throughput} & \textbf{Memory} \\
 &  &  & \textbf{(chars/sec)} & \textbf{(MB)} \\
\midrule
NUPunkt & 0.911 & 0.725 & 10M & 432 \\
CharBoundary (L) & 0.763 & 0.782 & 518K & 5,734 \\
CharBoundary (M) & 0.757 & 0.779 & 587K & 1,897 \\
CharBoundary (S) & 0.746 & 0.773 & 748K & 1,026 \\
spaCy (sm) & 0.647 & 0.657 & 97K & 1,231 \\
spaCy (lg) & 0.643 & 0.652 & 91K & 2,367 \\
NLTK Punkt & 0.621 & 0.708 & 9M & 460 \\
PySBD & 0.593 & 0.716 & 258K & 1,509 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/memory_usage_table.tex <==
\begin{table*}[htbp!]
\centering
\caption{Memory Usage of Sentence Boundary Detection Methods}
\label{tab:memory-usage}
\begin{tabular}{lrrrr}
\toprule
\textbf{Tokenizer} & \textbf{Init (MB)} & \textbf{Tokenize (MB)} & \textbf{Bulk (MB)} & \textbf{Total (MB)} \\
\midrule
NUPunkt & 229.72 & 200.89 & 202.43 & 432.15 \\
NLTK Punkt & 285.39 & 174.21 & 174.25 & 459.63 \\
spaCy (sm) & 540.52 & 431.77 & 690.55 & 1231.07 \\
spaCy (lg) & 1060.02 & 1053.47 & 1307.31 & 2367.32 \\
pySBD & 1076.31 & 432.29 & 432.75 & 1509.06 \\
CharBoundary\_small & 518.77 & 506.91 & 507.07 & 1025.84 \\
CharBoundary\_medium & 948.56 & 948.66 & 948.20 & 1896.75 \\
CharBoundary\_large & 3402.06 & 2331.57 & 2331.87 & 5733.93 \\
\bottomrule
\end{tabular}
\end{table*}



==> tables/precision_performance_table.tex <==
\begin{table*}[htbp!]
\centering
\caption{Sentence Boundary Detection Performance on Legal Texts by Dataset}
\label{tab:sbd-precision-performance}
\begin{tabular}{llrrrr}
\toprule
Dataset & Model & \textbf{Precision} & Chars/sec & F1 & Recall \\
\midrule
ALEA SBD Benchmark & NUPunkt & 0.918 & 10.00M & 0.842 & 0.778 \\
 & CharBoundary_large & 0.637 & 518.06K & 0.727 & 0.847 \\
 & CharBoundary_medium & 0.631 & 586.62K & 0.722 & 0.842 \\
 & CharBoundary_small & 0.624 & 748.36K & 0.718 & 0.845 \\
 & NLTK Punkt & 0.537 & 9.09M & 0.646 & 0.811 \\
 & spaCy (lg) & 0.517 & 90.93K & 0.572 & 0.640 \\
 & spaCy (sm) & 0.516 & 96.51K & 0.573 & 0.644 \\
 & pySBD & 0.468 & 258.37K & 0.627 & 0.948 \\
\midrule
SCOTUS & CharBoundary_large & 0.950 & 1.16M & 0.778 & 0.658 \\
 & CharBoundary_medium & 0.938 & 1.36M & 0.775 & 0.661 \\
 & CharBoundary_small & 0.926 & 1.35M & 0.773 & 0.664 \\
 & NUPunkt & 0.847 & 4.75M & 0.570 & 0.429 \\
 & spaCy (sm) & 0.825 & 110.13K & 0.761 & 0.706 \\
 & spaCy (lg) & 0.819 & 78.48K & 0.753 & 0.696 \\
 & pySBD & 0.799 & 284.47K & 0.817 & 0.835 \\
 & NLTK Punkt & 0.710 & 11.03M & 0.760 & 0.817 \\
\midrule
Cyber Crime & CharBoundary_large & 0.968 & 698.33K & 0.853 & 0.762 \\
 & CharBoundary_medium & 0.961 & 797.32K & 0.853 & 0.767 \\
 & CharBoundary_small & 0.939 & 806.91K & 0.837 & 0.755 \\
 & NUPunkt & 0.901 & 11.29M & 0.591 & 0.439 \\
 & spaCy (sm) & 0.842 & 106.00K & 0.776 & 0.720 \\
 & pySBD & 0.831 & 216.49K & 0.833 & 0.835 \\
 & spaCy (lg) & 0.830 & 94.07K & 0.769 & 0.717 \\
 & NLTK Punkt & 0.748 & 10.40M & 0.782 & 0.819 \\
\midrule
BVA & NUPunkt & 0.987 & 14.77M & 0.608 & 0.440 \\
 & CharBoundary_large & 0.963 & 991.14K & 0.881 & 0.813 \\
 & CharBoundary_medium & 0.957 & 1.25M & 0.875 & 0.806 \\
 & CharBoundary_small & 0.937 & 1.40M & 0.870 & 0.812 \\
 & pySBD & 0.795 & 217.58K & 0.857 & 0.929 \\
 & spaCy (sm) & 0.750 & 109.73K & 0.563 & 0.451 \\
 & spaCy (lg) & 0.720 & 114.30K & 0.554 & 0.450 \\
 & NLTK Punkt & 0.696 & 11.34M & 0.775 & 0.875 \\
\midrule
Intellectual Property & CharBoundary_large & 0.954 & 791.24K & 0.890 & 0.834 \\
 & CharBoundary_medium & 0.948 & 937.46K & 0.889 & 0.837 \\
 & CharBoundary_small & 0.927 & 980.53K & 0.883 & 0.843 \\
 & NUPunkt & 0.912 & 13.01M & 0.595 & 0.442 \\
 & spaCy (sm) & 0.852 & 91.09K & 0.802 & 0.757 \\
 & spaCy (lg) & 0.839 & 92.16K & 0.792 & 0.749 \\
 & pySBD & 0.829 & 255.15K & 0.860 & 0.894 \\
 & NLTK Punkt & 0.724 & 10.65M & 0.781 & 0.847 \\
\bottomrule
\end{tabular}
\end{table*}


